Rethinking Generic Object Tracking Toward Human-Level Perceptual Intelligence

At the heart of human visual perception lies the ability to maintain a continuous and coherent understanding of the external world. By integrating observations with accumulated experience, the human visual system can continuously adapt to variations in both the target and its surrounding environment, while preserving robust visual continuity as scene dynamics evolve. Human vision can therefore integrate prior knowledge, spatial geometry, and semantic context to understand complex scenes and their changes. As a core problem in computer vision, visual object tracking aims to bring machine perception closer to human visual perception. These capabilities are central to the task of Generic Object Tracking (GOT). In this task, a visual tracker is initialized only with the bounding box of an arbitrarily specified target in the first frame, and must continuously localize the target in subsequent dynamic visual streams. However, future events, observations, and real-world variations are inherently unpredictable; therefore, the model's generalization and online adaptation capabilities remain bottlenecks. Tracking reliability can deteriorate when the target undergoes severe deformation, is affected by complex distractors, encounters significant environmental changes, or belongs to a category unseen during training. This dissertation aims to narrow the gap between machine visual tracking systems and human visual perception by proposing a series of methods that systematically enhance the target discrimination, robust adaptation, and geometric reasoning capabilities of tracking models.

==> Abstracts/abstractCH.tex <==
% Removed in the English-only arXiv version.


==> Infos/acronyms.tex <==
%% The package Acronym can be used in the text like this %% 

%% blablablablabl \ac{CDMA} , it is the first time I am talking about CDMA. 
%% bloblobbloblob \ac{CDMA}, I already talked about CDMA. 
%% bliblibliblibli \acl{CDMA} for some reason I want to use the full name here. 

% \begin{acronym}

%% DEFINE ALL YOUR ACRONYMS HERE %%
% \acro{AR}{Augmented Reality}

  
% \end{acronym}

==> chapters/got_edit_chapters/3_Related_Work.tex <==

\section{Related Work}
\label{sec:GOT-Edit_Related_Work}



%%% less criticise matching-based tracker

% 2.1 GOT- match tracking by det
% point tracker
% why above fail, what we  have done


%%\vspace{-0.1in}
\paragraph{Generic Object Tracking.}  
%
Existing methods for Generic Object Tracking (GOT) task are typically derived from two pipelines~\cite{jav_got_survey}: 
matching-based trackers and tracking-by-detection trackers.
%
The matching-based paradigm formulates tracking as a similarity learning task followed by matching~\cite{SiamFC, SiamRPN, SiamCAR, SiamFC++, Siam_R-CNN, SiamAttN, Ocean, STARK, Learning_to_filter, TransT, OSTrack, TransInMo, ROMTrack, AiATrack, TATrack, RFGM, CiteTracker, SeqTrack, AQATrack, ARTrackV2, EVPTrack, HIPTrack, CTTrack, DropMAE, MAT, Diff-Tracker, DiffusionTrack, AsymTrack}.
%
These methods focus on training a deep network to learn a function that can distinguish and match a template of the object to a search region in the current frame.
%
This trained network is then used for tracking. 
%
Recent matching-based trackers~\cite{DreamTrack, LMTrack, MambaLCT, MCITrack, TemTrack} further improve their robustness by propagating chronological contextual information from predicted hidden states.

Another paradigm, tracking-by-detection, frames generic object tracking as an online detection task~\cite{bolme2010visual, hen_exploiting,MDNet, BACFgaloogahi, RTINet, lukezic2017discriminative, ECO, CCOT, HSET,RTAA}. 
Recent trackers under this paradigm employ a model predictor that generates a target-specific tracking model from paired reference images and labels, allowing more accurate object localization in the current frame~\cite{DiMP, ToMP, PiVOT}. 
%
The model predictor is dynamically updated for each incoming frame by referring to previous tracking results and hence enhances the tracker's robustness and adaptivity. 
%
A separate localization head then uses this updated model to pinpoint the target.

Despite progress in the above two paradigms, they remain limited by their reliance solely on two-dimensional spatial and structural knowledge.
%
To overcome this, our method integrates 2D semantic information with 3D geometric features, enabling a 2D tracker to exploit 3D geometry information through online tracking model editing.

%%\vspace{-0.15in}
%%%\vspace{-0.20in}



\paragraph{3D Features for Tracking.}
Existing trackers that utilize 3D features fall into two primary categories: those that augment RGB images with additional modalities (RGB+X)~\cite{Depthtrack,yang2022towards,ViPT,SDSTrack,BAT,FlexTrack,XTrack,SUTrack,CSTrack,STTrack} and those that operate directly on point cloud data~\cite{HVTrack,CUTrack,M3SOT,SCVTrack,SeMoLi,MITracker}. 
%
These approaches require auxiliary inputs during tracking, such as pre-computed depth maps or scene point clouds, which are generally unavailable in real-world scenarios where scenes and objects may be arbitrary and even previously unseen.
%
Another line of research~\cite{TAP-Vid,PIPs,TAPIR,OmniMotion,Cotracker,Chrono}, known as point tracking, explores tracking any pixel.
%
Recent extensions~\cite{SpatialTrackerV2,Tracktention,MVTracker,VGGT,AllTracker} incorporate 3D information for point tracking.
% , but their formulation remains pixel-level and cannot leverage object-level semantics, which are crucial for GOT.

Unlike these methods, our tracker adaptively integrates 3D geometric knowledge with 2D semantic knowledge for GOT through online model editing.
Specifically, we embed VGGT~\cite{VGGT} into a 2D tracker, where a sequence of RGB frames is used to derive complementary 3D information.
While geometric features from VGGT have proved effective for point tracking~\cite{VGGT,Cotracker}, our method departs from this line of work by embedding these features into a 2D GOT tracker via model editing, thereby establishing a direct connection between 3D geometric representations and object-level semantics for tracking.
%
In this way, our formulation operates directly on RGB streams and extracts geometric cues from them, yielding a geometry–aware and semantics–preserving GOT formulation that matches the intrinsic nature of the task and aligns with the way human observers infer scene structure from two-dimensional imagery.



% %%\vspace{-0.1in}


==> chapters/pivot_chapters/1_abstract.tex <==
Learning a discriminative model that distinguishes the specified target from surrounding distractors across frames is essential for generic object tracking (GOT). Dynamic adaptation of target representation against distractors remains challenging because prevailing trackers exhibit limited discriminative capability.
%
To address this issue, we present a new visual prompting mechanism for generic object tracking, termed PiVOT. PiVOT introduces mechanisms that leverage the pretrained foundation model (CLIP) to automatically generate and refine visual prompts online, thereby enabling the tracker to suppress distractors through contrastive guidance.
%
To transfer contrastive knowledge from the foundation model to the tracker, PiVOT automatically propagates this knowledge online and dynamically generates and updates visual prompts. Specifically, it proposes a prompt initialization mechanism that produces an initial visual prompt highlighting potential target locations. The foundation model is then used to refine the prompt based on appearance similarities between candidate objects and reference templates across potential targets. After refinement, the visual prompt better highlights potential target locations and reduces irrelevant prompt information.
%
With the proposed prompting mechanism, the tracker can generate instance-aware feature maps guided by the visual prompts, which are incrementally and automatically updated during tracking, thereby effectively suppressing distractors.
%
Extensive experiments across multiple benchmarks indicate that PiVOT, with the proposed prompting mechanism, can suppress distracting objects and improve tracking performance.
